Tests of subgrid models for star formation using simulations of isolated disk galaxies

We use smoothed-particle hydrodynamics simulations of isolated Milky Way-mass disk galaxies that include cold, interstellar gas to test subgrid prescriptions for star formation (SF). Our fiducial model combines a Schmidt law with a gravitational instability criterion, but we also test density thresholds and temperature ceilings. While SF histories are insensitive to the prescription for SF, the Kennicutt-Schmidt (KS) relations between SF rate and gas surface density can discriminate between models. We show that our fiducial model, with an SF efficiency per free-fall time of 1 per cent, agrees with spatially-resolved and azimuthally-averaged observed KS relations for neutral, atomic and molecular gas. Density thresholds do not perform as well. While temperature ceilings selecting cold, molecular gas can match the data for galaxies with solar metallicity, they are unsuitable for very low-metallicity gas and hence for cosmological simulations. We argue that SF criteria should be applied at the resolution limit rather than at a fixed physical scale, which means that we should aim for numerical convergence of observables rather than of the properties of gas labelled as star-forming. Our fiducial model yields good convergence when the mass resolution is varied by nearly 4 orders of magnitude, with the exception of the spatially-resolved molecular KS relation at low surface densities. For the gravitational instability criterion, we quantify the impact on the KS relations of gravitational softening, the SF efficiency, and the strength of supernova feedback, as well as of observable parameters such as the inclusion of ionized gas, the averaging scale, and the metallicity.

==> best_model.tex <==

\subsection{Star formation history and birth densities}
Besides the KS relation we will also show the impact the criteria and laws have on the SFH and birth densities. 


==> ionized.tex <==
\subsection{Importance ionized gas}
In this subsection we show that especially at low surface densities in Fig. \ref{fig:importance-HII} ionized gas is important in terms of the total surface density, and therefore not taking into account the total surface density; $\Sigma_H = \Sigma_{\rm HII} + \Sigma_{\rm HI} + \Sigma_{\rm H_2}$ but for example only $\Sigma_{\rm HI} + \Sigma_{\rm H_2}$ will have an impact at low surface densities. This especially if you look at Fig. \ref{fig:KS-importance-HII} will cause your KS relation to have a stronger break compared to when you do take into account ionized gas, therefore it is important to compare observations and simulations on equal grounds. 

\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/importance_ionized_gas_0500.png}
    \caption{Fraction of gas that is not ionized for a specific surface density}
    \label{fig:importance-HII}
\end{figure}
\end{comment}



==> observed_SFE.tex <==
\subsection{Constant efficiency does not imply constant SFE}

\citet{ellison2020} showed that their ALMaQUEST sample of galaxies shows that a difference from the main sequence of the star formation $\Delta \Sigma_{SFR}$ is mainly due to a difference in the SFE, we show that on observational scales this indeed can be observed, but that this does not imply that on scales not resolved by the observations the SFE is varying with local properties, we show that a model with constant SFE can cause the same correlation. See Fig. \ref{fig:correlation-SFE}.

\begin{figure}
	\includegraphics[width=\columnwidth]{figures/Correlation_plot_0100.png}
    \caption{}
    \label{fig:correlation-SFE}
\end{figure}

==> old_stuff.tex <==


%Our work is not the first attempt to understand the SF scaling relations better in hydrodynamical simulations. There have been many works on SF however most of these works are using an equation of states (EoS) that prevent the gas to cool down to low temperatures, $T<10^3~\rm K$ \citep[e.g.][]{springel2003,stinson2006,schaye2008}. Because gas is not allowed to cool down to lower temperatures, gas is smoothed on the \citet{jeans1902} length that typically is around $1~\rm kpc$. This means that at a fixed galactic radius the density is almost constant, therefore, the spatially-resolved and azimuthally averaged KS relations will be very similar while this is not true for simulations with a cold phase like ours. \citet{marinacci2019} and works based on this model \citep{sivasankaran2022,jahn2021} showed that there are significant differences between hydrodynamical simulations with and without an EoS. The differences are expressed in more variation of the SFH on time scales of $t\sim 20~\rm Myr$ and a larger scatter in the $\Sigma_{\rm SFR}$ at fixed gas surface densities. Because of these effects, we only compare our results with simulations that explicitly model the cooling to cold gas ($T<10^2 ~\rm K$).
\begin{comment}
\subsubsection{FIRE models}

\citet{hopkins2013} used idealised disk galaxies to investigate the impact that different SF criteria have on the total SFR of galaxies. They investigated several different criteria, i.e. temperature threshold, Jeans instability, converging flows, $t_{\rm cool}<t_{\rm ff}$ and instability criterion. They found that the SFHs are almost identical (their fig. 1). \citet{hopkins2014} showed that the FIRE model with an instability criterion, high-density criterion ($n_{\rm H} > 10^2~\rm cm^{-3}$), and 100 per cent SFE is able to match the galaxy-averaged KS relation. \citet{orr2018} also investigated the spatially-resolved KS relation in the FIRE simulation and found that the scatter of the KS relation is well reproduced. The slopes they obtained (from their fig. 2) are a bit higher $N\approx 1.7$ than observed. They found that the normalisation of the molecular KS relation is around 1.5 dex too high (their fig. 2), similar to what we find when increasing the SFE. \citet{hopkins2018} showed in their fig. 34 that the exact SF criterion and SFE do not impact the SFH of an MW-mass galaxy, in agreement with our Fig. \ref{fig:KS-crits}. \citet{hopkins2022} looked at the density distribution of star-forming gas and find that the high-density criterion $n_{\rm H}>10^3~\rm cm^{-3}$ can produce artificial features at the corresponding density (their fig. 6). Therefore, they concluded that it is better to use an instability criterion.

%They focused on an instability criteria, a density criteria ($n_{sf}>100~\rm cm^{-3}$), a criteria that all molecular gas is star-forming, a temperature criteria ($T_{\rm crit}<10^2~ \rm K$), a Jeans instability criterion, gas with $\nabla \cdot \mathbf{v}<0$ is star-forming, and gas is star-forming when $t_{\rm cool}<t_{\rm dyn}$. Similar to us, they found that independent of the SF criterion used, the SFR is very similar. \citet{hopkins2014} showed that the Fire model with a combined SF criterion of an instability criterion and a density criterion ($n_{\rm H} > 10^2~\rm cm^{-3}$) together with an efficiency of 100 per cent is able to match the galaxy-averaged KS relation from halo masses of $1.9\times 10^9$ to $10^{13}$. \citet{orr2018} found that the scatter of the KS relation is well reproduced in the Fire2 simulation, the normalisation of the molecular KS relation is around 1 dex too high for their galaxies. They find that the molecular KS relation does not change significantly when the spatially-resolved bin sizes are changed from 0.1 kpc to 1 kpc. This seems inconsistent with our result, but they only look at this for higher surface densities $\Sigma_{\rm H_2} > 1~\rm M_\odot ~\rm pc^{-2}$. In our simulations, the differences above this surface density are also very small. Our model with an SFE of 100 per cent has a similar offset of the molecular KS relation of around 1 dex, so our results are consistent with what \citet{orr2018} found. \citet{hopkins2018} showed that in the Fire 2 model the exact numerical implementation of the SF criterion is not important in an MW-mass galaxy, in agreement with what we find. Their default model includes an instability criterion, density criterion and Jeans instability criterion. As shown in \S \ref{subsub:instability} a Jeans instability criterion and an instability criterion are the same. \citet{hopkins2022} looked at the density distribution of star-forming gas and find that the high-density criterion $n_{\rm H}>10^3~\rm cm^{-3}$ is the most important in determining the density distribution of the gas. When no high-density criterion is used the instability criterion sets the density distribution.

\subsubsection{Models with AREPO}
Using the moving mesh code AREPO \citep{springel2010}, \citet{marinacci2019} presented the SMUGGLE subgrid model that includes many subgrid processes. Among other runs, they modelled isolated disk galaxies that include the same feedback processes as in our simulations. For the azimuthally-averaged KS relation they found a slope of around $N\approx 4$ to $6$ depending on the resolution (their fig. 4), where we find that the azimuthally-averaged KS relations have a constant slope that is similar to $N\approx 1.4$. \citet{li2020} showed that varying the SFE does not change the SFR significantly between 1 per cent and 100 per cent (their fig. 2), similar to what we find.  

Using a different subgrid model, \citet{gensior2020} used the SFE that depends on the virial parameter they found that the slope of their azimuthally-averaged KS relation is $\approx 2.5$ (their fig. 3) steeper than our simulation and than observed.

%They compared their simulated azimuthally averaged KS relation and show that there is a clear break in the KS relation. Rather than the trend of a slope similar to the observed relation they find a slope that is steeper. \citet{li2020} found that varying the SFE does not change the SFR significantly between 1\% and 100\%. However, they find that initially a higher (lower) SFE produces a slightly higher (lower) SFR initially and later in the simulation this produces a lower (higher) SFR.

\subsubsection{Semenov models}
%\citet{gnedin2011} showed that they get a slight difference in normalisation for the KS relation for different density thresholds and that their slope is slightly steeper when the density threshold.

Using the adaptive mesh refinement (AMR) code ART \citep{kravtsov1997}, \citet{semenov2016} adopted an SF efficiency that depends explicitly on the boundedness of the gas with a subgrid model for turbulence. They found good agreement with the spatially-resolved KS relation (their fig. 4) and have a slope around $N\approx 1.4$ at high surface densities. Similarly, \citet{semenov2017} showed that using an instability criterion for SF results in a good fit to the spatially-resolved neutral KS relation with slopes in agreement with ours. They found that the normalisation for the molecular KS relation is 0.5 dex to high. \citet{semenov2018} showed that as long as $\varepsilon \ga 0.01$ the global depletion time of the simulation will self-regulate (their fig. 2), we find agreement with this but find that even for $\varepsilon=0.001$ the global SFR is relatively similar.

%\begin{comment}
\citet{semenov2019} did simulations using different slopes in the SFR ranging from 1 to 2.5 (where 1.5 is the fiducial \citet{schmidt1959} law) and find the spatially-averaged KS relations are insensitive to the slope of the small scale SF law. Therefore, we expect that our results are also robust for different SF laws. \citet{semenov2021} showed that the depletion time for different measured scales forms a wide tuning fork as expected from the SF uncertainty principle, they demonstrated that the adopted parameters to convert to observations are impacting the result largely. We find that for different spatially averaging time scales the KS relation changes similar to the SF tuning fork and is more straightforward to measure.
%\end{comment}



%Their simulations have a much stronger spiral arm structure that might be related to the fact that they are using AMR instead of an SPH-based scheme.
%\citet{semenov2018} showed that as long as $\varepsilon>0.01$ the global depletion time of the simulation will self-regulate.
%\citet{semenov2019} did simulations of SF models with different slopes ranging from $1$ to $2.5$ instead of the fiducial $1.5$ for the \citet{schmidt1959} law. They found that when including feedback this produces an almost identical global depletion time and their results show similar behaviour for $\varepsilon=0.01$ and $\varepsilon=1.0$. \citet{semenov2021} showed the depletion time for different measured scales forms a wide tuning fork. This tuning fork is sensitive to the different adopted parameters in the SF model. However, they also show that the tuning fork is very sensitive to the applied observational cuts.

%\begin{comment}
\subsubsection{NIHAO models}
Here we discuss some results based on the NIHAO simulations \citep{wang2015} that are based on the \citet{stinson2006} SF model. \citet{dutton2019} showed that on short time scales the scatter in the SFR is smaller when a lower density threshold is used (their fig. 13), similar to what we find for weaker SF criteria. \citet{buck2019} looked at different density criteria for SF and proposed to use the cluster strength of newly formed stars to determine which SF models are better. \citet{dutton2020} showed in their fig. 6 that a lower density threshold will have a lower clustering amplitude and longer correlation length. This implies that a lower density threshold has a less pronounced break in the KS relations. %This implies that the KS relation has a break at higher surface densities in agreement with what we find.
%\end{comment}

\subsubsection{Models in Enzo}
Using the AMR code ENZO \citep{bryan2014}, \citet{becerra2014} investigated the impact of different density criteria on the total KS relation, they found that with higher density criteria the normalisation of the total KS relation is increased. This is in agreement with what we are finding, higher density criteria form stars at higher surface densities and correspondingly have a slightly lower $\Sigma_{\rm SFR}$. They also found good slopes for the KS relation. Similar to us, they found that increasing the SFE does not influence the slope but increases the normalisation of the neutral KS relation above $\Sigma_{\rm \ion{H}{I} + H_2}=3~\rm M_\odot ~\rm pc^{-2}$. Furthermore, they investigated the impact of binning size on the spatially-resolved total KS relation and find, similar to us, that the slope remains almost identical for binning sizes of 0.5 kpc to 10 kpc. For bin sizes of 0.1 kpc they find a slope that is close to 0.4. This is slightly in disagreement with what we are finding but they did not include non-detections in their relations, which could explain the difference.

%\begin{comment}
\citet{oh2020} also did simulations with ENZO with a different subgrid model and investigated different parameters for the SFE, they find in general that their KS relation is too steep and produces slopes of around $N\approx 5$ (their fig. 6).
%\end{comment}

\subsubsection{GADGET KROME model}
Using the improved \citet{beck2016} SPH scheme in Gadget3 \citep{springel2005b} with the non-equilibrium chemical network KROME \citep{grassi2014}, \citet{sillero2021} compared a density threshold with an instability criterion. They found that the SFR and morphology of the galaxies are nearly identical. Furthermore, they show that their spatially-resolved KS relation is very similar for both criteria and has a slope of around $N\approx 1.4$ in agreement with observations. They also show that the atomic KS relation is much steeper $N\approx 4$ than the neutral and molecular KS relation. This is similar to what we find but our slope is less steep, $N\approx 3$.

%an SF model that uses a constant SFE ($\varepsilon=0.1$) and molecular gas SF criterion with a model that uses a viral parameter-dependent SFE. They found that the SFR and morphology of the galaxies are nearly identical. However, they showed that the exact location of SF is different for both methods --- the stricter (milder) criterion selects smaller (larger) high (low) density regions that form stars.

%\begin{comment}
\subsubsection{Grisdale models}
\citet{grisdale2021} compared a density-temperature criterion with an instability criterion and found that the SFR is very similar. Furthermore, they did not find any difference in the KS relations for both SF criteria.
%\end{comment}

%\begin{comment}
\subsubsection{Gasoline models}
Using GASOLINE \citep{wadsley2004}, \citet{christensen2014} used the SF model of \citet{stinson2006} with a density ($n_{\rm H}=10 ~\rm cm^{-3}$) and temperature threshold ($10^4~\rm K$). They showed that their neutral KS relation agrees with the \citet{bigiel2008} data at low surface densities. However, they do not investigate surface densities beyond the break.  
%\end{comment}

\subsubsection{Ramses models}
Using the AMR code RAMSES \citep{teyssier2002}, \citet{agertz2013} investigated an SF model in isolated disk galaxies using a metallicity-dependent density criterion and a temperature criterion of $10^4~\rm K$. They showed in their fig. 12 that their resolved KS relation agrees for 1 per cent SFE while for 10 per cent it overshoots the normalisation of the KS relation identical to what we find. Furthermore, they showed that their implementation is sensitive to the exact feedback scheme that is used and can alter the normalisation and the breakpoint (their fig. 13). \citet{agertz2015} investigated the resolved KS relation for a cosmological simulation. In general, they found that their slope at high surface densities $\Sigma_{\rm \ion{H}{I} + H_2} > 10^1~\rm M_\odot ~\rm pc^{-2}$ is more steep and has a slope of $N\approx 2.5$ (their fig. 11) instead of the observed $N\approx 1.4$ \citep{kennicutt1998}.

\subsubsection{Lessons learned}
\textcolor{red}{Add a subsections lessons learned!}

\end{comment}
%However, using adaptive gravitational softening is computationally expensive and at small softening scales it will cause two-body scatter in cosmological simulations \citep[see][]{ludlow2020}, we do not use adaptive gravitational softening in this work. This means that the self-consistent collapse of gas is limited by $M_{\rm particle}/\epsilon^3$ corresponding to $n_{\rm H} = 0.4~\rm cm^{-3}$. This means that strict criteria have the problem of an inconsistent collapse at higher densities. In Fig.~\ref{fig:KS-grav-sof} three simulations with different gravitational softening lengths show that the impact on the KS relation is small and therefore the use of smaller gravitational softening scales is not justified.


==> selection.tex <==
\subsection{Phase space selection of star forming gas}

In Fig. \ref{fig:SF-TnH} we show the fraction of gas particles that are clasified as star forming in the \texttt{fid} simulation that uses the virial criterion. We see that the virial criterion mainly selects gas in the highest density regions above $10^2~\rm cm^{-3}$. Compared to both temperature criteria (i.e. $10^2$ and $10^3~\rm K$) this means that the virial criterion selects way less gas that is at very low densities (i.e. $<1~\rm cm^{-3}$) this as a consequence has that the virial criterion will therefore selects gas in higher density regions and therefore target spiral arms more (see below). Because the virial criterion scales as $\alpha_{\rm vir} \propto \rho^{-1/3}$, this means that at higher densities the virial criterion is able to select gas that has a higher than the temperature criteria. 

\begin{figure}
	\includegraphics[width=\columnwidth, trim={0 1cm 0 1.5cm}, clip]{figures/fraction_SF_phase_space_0100_fid.png}
    \caption{Comparison of the density temperature space that the virial criterion selects compared to a temperature criterion. \textcolor{red}{Add 2 lines for $10^2$ and $10^3$ K to compare with these models which gas is selected, this figure needs better colorbar (too long)}}
    \label{fig:SF-TnH}
\end{figure}


\subsection{Spatial selection of star forming gas}

In Fig. \ref{fig:SF-gas-spatially} we show for the \texttt{fid} and \texttt{T1e3K} run the gas that is selected to be star forming in both simulations. In the top panel of Fig. \ref{fig:SF-gas-spatially} we see the face-on view of the galaxy and the SFR surface density in the galaxy, it is clear that the virial criterion on the left selects gas more thinly while the temperature criterion selects more gas at lower densities that also correspond regions with lower surface densities. In the bottom panel of Fig. \ref{fig:SF-gas-spatially} we show the edge on view of both criterion and we can see that \texttt{fid} selects only gas that is very close to the midplane of the disk galaxy, while \texttt{T1e3K} selects gas up to higher vertical distances from the midplane. From this it becomes apparent that \texttt{fid} which selects based on the virial criterion is able to more realistically select star forming regions. 
 
\begin{figure}
	\includegraphics[width=0.48\columnwidth, trim={4.55cm 0 0 0}, clip]{figures/project_star_formation_rates_0100_fid.png}
	\includegraphics[width=0.48\columnwidth, trim={4.55cm 0 0 0}, clip]{figures/project_star_formation_rates_0100_T1e3.png}

    \caption{Comparison between gas selected to be star forming between the virial criterion (left) and a temperature criterion (right). Top: face-on view of the gas that is star forming, bottom: edge on view of the gas that is star forming. \textcolor{red}{Improve by adding criterion name in image, make edge-on smaller (10 kpc height would do), single image}}
    \label{fig:SF-gas-spatially}
\end{figure}

==> star_formation_models.tex <==

\begin{comment}
\subsection{Star formation models}
In hydrodynamical simulations of galaxies it is not possible to resolve the complete scale of star formation, because of this it is required to have a subgrid model for star formation that describes when and at which rate gas particles form stellar particles. In this section we will explain the two main components of the star formation subgrid model, the star formation rate and when gas is star forming. 


\subsubsection{When is gas forming stars?}
We need to determine which gas is star forming, in order to do this we need to have a criteria that tells us when gas becomes star forming in this paper we will focus on two criteria the temperature criterion and the instability criterion. before we look at both of these criteria we also impose a few additional criteria on the gas in order to form stars, firstly we require the gas to have a high enough over density above the cosmic mean baryon density in order to prevent star formation in low density regions:
\begin{align}
    \rho_g > \Delta_{\rm SF} \Omega_{\rm b} \rho_{\rm c}.
\end{align}
In which we take $\Delta_{SF}=57.7$ following \citet{schaye2008}. Besides this we explicitly impose that gas particles that are hosting a HII region cannot form stars. 


\subsubsection{Temperature criterion} 
The first type of criterion is a temperature criterion, selecting only gas that is cold:
\begin{equation}
    T_{\rm subgrid} < T_{\rm crit.}.
\end{equation}
In which $T_{\rm crit.}$ is a temperature low enough to only select gas that is expected to have conditions to form stars. In Fig. \ref{fig:TnH-criteria} we can see that the equilibrium cooling lines at solar metallicity and 10\% solar metallicity will select gas at low densities that can cool down. We note that due to tidal forces in the galaxy the temperature of the gas can be slightly higher than the equilibrium cooling curve indicates, this means that a temperature criterion might not work ideally at especially low metallicities, in order to prevent this it is required to include an additional criterion for low metallicity gas. The simplest solution for this is to also include an additional density criterion, which means that when the gas does not satisfies the temperature criterion it is star forming when it forms the density criterion, $n_H > n_{H, \rm crit.}$. We choose to set the value of $n_{H, \rm crit.}= 10^3~\rm cm^{-3}$, which is around the density at which the primordial gas goes below the critical temperature.

\subsubsection{Instability} %Folkert
The argument for the virial criteria is that gas is only allowed to form when the gas is locally bound and unstable such that we would expect gas to 
collapse. This basically means that we want a general Jeans equation in which the pressure of the cloud competes with the gravitational force that wants to collapse the cloud, therefore in order for a cloud to collapse it is required that $t_{\rm ff} < t_{sc}$, in which we have:
\begin{align}
  t_{\rm sc} &= \frac{R}{\sqrt{\sigma_{\rm th}^2 + \sigma_{\rm turb}^2}}.
\end{align}
Taking into account the contribution from the thermal velocity dispersion and the turbulence velocity dispersion, other contribution can be added to the velocity dispersion. In which the thermal velocity dispersion is given by:
\begin{align}
    \sigma_{\rm th}^2 &= 3 \frac{P}{\rho} = \frac{3 k_B T}{\mu m_H}. 
\end{align}
and the turbulence velocity dispersion is calculated as:
\begin{equation}
    \sigma_{\rm turb}^2 = \frac{1}{\rho_i} \sum\limits_{j=1}^N m_j W(r_{ij}, h_i) |\mathbf{v}_i - \mathbf{v}_j|^2.
\end{equation}
Than the free-fall time is given by:
\begin{align}
    \tau_{\rm ff} = \sqrt{\frac{3\pi}{32 G\rho}}.
\end{align}
We can combine this to make a general Jeans length as:
\begin{align}
    \lambda_{\rm J} = \sqrt{\frac{3\pi(\sigma_{\rm th}^2 + \sigma_{\rm turb}^2)}{32 G \rho}}.
\end{align}
We can than construct a general Jeans mass, $M_J = \frac{4\pi}{3}\rho \lambda_J^3$:
\begin{align}
    M_{\rm J} = \frac{4\pi}{3} \left( \frac{3\pi}{32}\right)^{3/2} \left( \frac{\sigma_{\rm th}^2 + \sigma_{\rm turb}^2}{G} \right)^{3/2} \rho^{-1/2}.
\end{align}
When the Jeans mass is smaller than the resolution mass the gas particles are assumed to be star forming:
\begin{align}
    M_{\rm J} < M_{\rm res} = \langle N_{\rm ngb} \rangle M_{\rm particle}.
\end{align}
This means we get an expression given by:
\begin{align}
    \alpha \equiv \frac{\sigma_{\rm th}^2 + \sigma_{\rm turb}^2}{G \langle N_{\rm ngb} \rangle^{2/3} M_{\rm particle}^{2/3} \rho^{1/3}} < \alpha_{\rm vir.}
\end{align}
In which lower values of $\alpha_{\rm vir.}$ mean the cloud is more gravitationally bound, our default case is using $\alpha_{\rm vir.}=1$. We note that in the case of having $\sigma_{\rm turb}^2$ we have a criterion that is almost identical to a Jeans instability criterion. A criteria like this have been used before in hydrodynamical simulations, like in \citet{hopkins2014, hopkins2018} and \citet{semenov2016} but the calculation of the virial criterion presented in this paper is not identical to the ones in these papers. 



\begin{figure}
	\includegraphics[width=\columnwidth]{figures/March_30_Equilibrium_temp.pdf}
    \caption{Temperature vs density plane in the region where we expect star forming gas to form, the gray lines indicate the equilibrium temperature of the cooling tables at different metallicities.}
    \label{fig:TnH-criteria}
\end{figure}
\end{comment}


\subsubsection{The star formation rate}
When gas is selected that forms stars, the star formation rate of the gas needs to be determined, in this paper we consider two different approaches the Schmidt law and pressure law.

\subsubsection{Schmidt law}
The Schmidt law assumes that the star formation rate depends on both the density and the free fall time as:
\begin{equation}
    \dot{\rho}_\star = \varepsilon \frac{\rho}{\tau_{\rm ff}}.
\end{equation}
In which $\tau_{\rm ff}$ is the free fall time given by:
\begin{align}
    \tau_{\rm ff} = \sqrt{\frac{3\pi}{32 G\rho}}.
\end{align}
This means that in a single free fall time the fraction $\varepsilon$ of the 
gas is converted into stars. Typical values for $\varepsilon$ range from 1\% 
to 100\% and in most simulations $\varepsilon$ is assumed to be constant. 
Recently there have been some models that vary the efficiency of the Schmidt
law by making the star formation efficiency depend on turbulance in the medium \citep{semenov2016}. In this paper we choose to have a constant $\varepsilon$. 

\subsubsection{Pressure law}
A second method is using a pressure law instead of a schmidt law. 
In a pressure law the star formation scales with the pressure instead of 
with the density \citep{schaye2008}:
\begin{equation}
    \dot{\rho}_\star = A \left( 1 \rm M_\odot \rm pc^{-2} \right)^{-n} \left( \frac{\gamma}{G} f_g P \right)^{(n-1)/2} \rho.
\end{equation}
In which $A$ is the normalization of the Kennicutt-Schmidt relation, $n$ is the
slope of the KS relation, $\gamma$ is the ratios of specific heats, $f_g$ is the 
gas fraction and $P$ is the pressure of the gas. In this case the star formation law
is constructed to explicitly reproduce the Kennicutt-Schmidt law \citep{kennicutt1998,kennicutt2021}. 

\begin{figure}
	\includegraphics[width=\columnwidth]{figures/log_depletion_time.png}
    \caption{The gas depletion time as a function of hydrogen density for the different models of star
formation. In this figure we show the theoretical lines for the pressure law for a temperature of 10 K
(dashed gray), 100 K (dashed yellow) and 1000 K (dashed cyan) and for the predictions of the Schmidt
law for all temperatures (dashed pink).}
    \label{fig:TnH-criteria}
\end{figure}

\begin{comment}
\subsection{Which gas is star forming?}
From observations of the Kennicutt-Schmidt law \citep{bigiel2008,Schruba2011} 
it is known that star formation becomes less efficient at low surface
densities between $\Sigma_{\rm gas} = 3 ~\rm M_\odot \rm pc^{-2}$ and 
$\Sigma_{\rm gas} = 10~ \rm M_\odot \rm pc^{-2}$. This means that not all
the gas in galaxies is star forming, because if all the gas would be 
star forming the Kennicutt-Schmidt relation would not have a break but 
extend until very low surface densities. 

Because not all the gas is star forming, gas in simulations needs to be 
selected based on a criteria to determine if gas is star forming. 
A common approach is to use a density threshold, that says that all the
gas above the density threshold is always star forming. In the literature
there have been a lot of differences in the value of the density threshold,
varying from $0.1 \rm cm^{-3}$ \citep{schaye2015} up to
$1000 \rm cm^{-3}$ \citep{hopkins2018}. Despite that a
density threshold is common practice in the literature it is not a very
satisfying criteria because there is no physical motivation to argue
that all the gas above the density threshold should be star forming. 
Especially in the case that there are SNII and HII regions that heat 
the ISM. This will cause gas that recently got ionized by a HII region
or recently hit by a SNII be still star forming, which is undesirable. 
In Fig. \ref{fig:selection_criteria} it can be seen that a density criteria
of around $n_H \sim 1~\rm cm^{-3}$ selects a large part of the gas at a 
temperature close to $10^4~ \rm K$. This in general would be argued to 
be undesirable.

\begin{figure}
	\includegraphics[width=\columnwidth]{figures/phase_space_criteria.png}
    \caption{Typical phase space diagram in a galaxy in which we see 
    4 lines for different criteria. Red: density threshold, Blue: 
    temperature threshold, cyan: Jeans criteria, orange: virial 
    criteria.}
    \label{fig:selection_criteria}
\end{figure}

A more physical motivated criteria is that stars only can form in cold 
gas. This means that we are using a temperature threshold. In the case 
that the cooling model can cool down to temperatures of around $10~\rm K$,
a temperature threshold is a good model. 

Despite that a temperature threshold will do better than a density threshold,
using a temperature threshold on its own is not the requirement for a gas 
cloud to start collapsing and form stars. For this we need to see if the 
free fall time is shorter than the sound crossing time, for this we basically
need to determine if gas is Jeans unstable. Given that a Jeans instability is 
hand waving argument we will set all coefficients to 1 for simplicity,
in this case the sound crossing time is given by:
\begin{equation}
    t_{\rm sound} = \frac{R}{c_s}.
\end{equation}
and the free fall time can be written as:
\begin{equation}
    t_{\rm ff} = \frac{1}{\sqrt{G\rho}}.
\end{equation}
If we combine both timescales, we can obtain a characteristic length scale 
above which all the gas is unstable for gravitational collapse, called the 
Jeans length:
\begin{equation}
    \lambda_J = \frac{c_s}{\sqrt{G\rho}}.
\end{equation}
We can convert a Jeans length into a corresponding mass above which gas goes
unstable, called the Jeans mass:
\begin{align}
    M_J &\equiv \rho \lambda_J^3 = \left( \frac{\gamma k_B T}{\mu m_H G} \right)^{3/2} \frac{1}{\sqrt{\rho}}, \\
    &= 2.1 \cdot 10^4 \text{M}_\odot \left( \frac{T}{100~\text{K}} \right)^{3/2} \left( \frac{n_H}{1~\text{cm}^{-3}} \right).
\end{align}
Assuming that $X=0.739$ and $\mu = 1.3$. From this it becomes clear that a 
Jeans criteria can be written effectively as a temperature criterion as:
\begin{equation}
    T \leq 100 \rm K \left( \frac{M_{res}}{2.1 \cdot 10^4 \rm M_\odot} \right)^{2/3} \left( \frac{n_H}{1~\text{cm}^{-3}} \right)^{1/3}.
\end{equation}
As can be seen this criterion has a resolution dependence and the normalization
of this relation depends on approximations used in the derivation. As can be 
seen from this relation the difference with respect to a temperature criteria
is only the slope and the normalization is very similar. We also note that the
normalization of a Jeans criterion is partly free to cho0se given that the 
coefficients in the free fall time, sound crossing time and other parts of the 
calculation can be chosen partly freely. Because of this the 
behaviour of a Jeans criterion is very similar to a simpler temperature
criterion as can be seen in Fig. \ref{fig:selection_criteria}, because of 
this there is a marginal difference between a 
temperature criterion and a Jeans criterion and therefore we will focus on 
the simpler temperature criterion for the remaining of this paper. 

The Jeans criterion only takes into account the gravitational interaction and 
the sound speed. In reality the sound crossing time should be calculated with
all the velocities in the molecular cloud:
\begin{equation}
    v^2 = c_s^2 + \sigma^2 + v_{B}^2 + \dots.
\end{equation}
In which $\sigma$ is the velocity dispersion, $v_{B}$ contributions from the
magnetic velocities and other contributions to this velocity. In our case we 
will only consider the sound velocity and the velocity dispersion as being part
of a more general Jeans criterion. In this case we take into account the most 
important contribution to the velocity but strictly speaking we only have an 
upper limit on whether the gas is star forming or not. This type of criteria 
is often called a virial criterion \citep{hopkins2013, hopkins2018} and 
means that the sound crossing time reduces to:
\begin{align}
    t_{\rm sound} = \frac{R}{\sqrt{c_s^2 + \sigma^2}}.
\end{align}
In which we now have the velocity dispersion in the sound crossing time. 
Using the same approach as for the Jeans criterion, we can write the 
virial criterion to a virial mass as:
\begin{align}
    M_J &=\left( \frac{\sigma^2 + c_s^2}{G} \right)^{3/2} \rho^{-1/2}.
\end{align}
This means that we can write this in terms of a simple criterion which
determines if gas is star forming or not as:
\begin{align}
    \alpha \equiv \frac{\sigma^2 + c_s^2}{G \rho^{1/3} M^{2/3}} < 1.
\end{align}
The selection of a virial cirterion in phase space is more difficult 
to visualize in Fig. \ref{fig:selection_criteria}, because a virial 
cirerion select more strictly gas than a Jeans criterion but it mainly
selects more on the dynamical properties, which is not done in the 
case of a Jeans criterion. This means that a virial criterion will
select more gas in regions that have a lower velocity dispersion.
This means that a virial criterion will be more closely selection 
gas around spiral arms as compared to a temperature criterion.

In the literature there have been several approaches to calculate the 
local velocity dispersion. In \citet{hopkins2014} they use the 
divergence and rotation of the velocity field to estimate the velocity
dispersion:
\begin{equation}
 \sigma^2 = (|\nabla \times \mathbf{v}|^2 + |\nabla \cdot \mathbf{v}|^2 ) h^2
\end{equation}
an other approach is to calculate the velocity gradient tensor and than 
calculate the Frobenius norm to calculate the velocity dispersion:
\begin{align}
    \sigma^2 &= \|\nabla \otimes \mathbf{v} \|_F h^2
\end{align}
\end{comment}



\begin{comment}
\subsubsection{Criteria and equation of states}
In the case of having a equation of state that limits the temperature
we cannot simply use the hydrodynamical temperature to determine if 
gas is star forming, for this we need to calculate a subgrid temperature.
A subgrid temperature is calculated assuming that the gas is in 
pressure equilibrium, this allows us to calculate the subgrid temperature 
and subgrid density for arbitrary densities and temperatures, then we find
the density and temperature that have the same pressure but are on 
the equilibrium density temperature line. In general we calculate the 
subgrid properties of the gas when it is sufficiently close to the 
equation of state, within $0.5$ dex.

In the case of the virial criterion we also use a subgrid density and 
subgrid temperature when gas is close to the equation of state and the 
sound speed is scales such that it uses the subgrid temperature instead
of the hydrodynamical temperature. 

\subsection{Forming stars in the simulation}
In our simulations we assign star formation rates to gas particles, but
we do not form a star particle for every star formation rate of a gas 
particle. Instead we use a probalistic approach to form stars in which 
every time step we calculate the probability of a gas particle to convert
to a star particle:
\begin{align}
    \rm Prob. &= \rm min \left( \frac{\dot{m}_\star \Delta t}{m_g}, 1 \right)
\end{align}
Then we draw a random number from a random number generator and check if 
the drawn random number $R$ is smaller or equal to the probabilty. If this 
is the case we will convert the gas particle immediately to a star particle.

\end{comment}

\begin{comment}
\subsection{Varying the Equation of State}
Most simulations of galaxy formation have a limited resolution, 
this limited resolution prevents these simulations to resolve the 
ISM structure properly. In these simulations it is common practice
to use a equation of state that limits the temperature of the simulation.
In which the temperature does not cool down below the equation of state.
Often these equation of states are temperature floors that depend on 
density. The current literature of galaxy formation follows either \citet{schaye2008} 
or \citet{springel2003}, in this paper we will follow the approach of 
\citet{schaye2008} by fixing an equation of state. 

Besides the limited resolution, there are two other reasons to use an
equation of state: Firstly, if the adopted cooling model does not 
take into account a cold phase a equation of state is required below 
the temperatures the cooling model is not working properly. Secondly,
using an equation of states prevents gas to cool down to high densities
which means that the simulation time of the simulation is reduces when
using an equation of state, because high density gas has shorter time 
steps and therefore increases the run time of the simulation.

In this work we will look at the impact of different equation of states 
on the star formation model. We will look at 4 different equations of 
states and runs without an equation of state. In our runs we will not 
impose the equation of state in temperature but rather in internal energy,
we do this because for a constant mean molecular weight both approaches
will give the same result, but for varying mean molecular weights, for 
example when gas transitions from molecular to neutral hydrogen or from
neutral to ionized a temperature equation of state will change the
Jeans length or Jeans mass of the gas with respect to an internal energy
equation of state.

% Example table
\begin{table}
	\centering
	\caption{The different equation of states used in this work}
	\label{tab:example_table}
	\begin{tabular}{lcccc} % four columns, alignment for each
		\hline
		Name & Jeans mass & Jeans length & slope & $T(0.1\rm cm^{-3})$ \\
		\hline
		high EoS & $4.8 \cdot 10^7 \rm M_\odot$ & $2400 \rm pc \left( \frac{n_H}{0.1 \rm cm^{-3}} \right)^{-1/3}$ & $1/3$ & 8000 K\\
		low EoS & $6.6 \cdot 10^4 \rm M_\odot$ & $270 \rm pc \left( \frac{n_H}{0.1 \rm cm^{-3}} \right)^{-1/3}$ & $1/3$ & 100 K\\
		EoSL100 & $3.3\cdot 10^3 \rm M_\odot \frac{n_H}{0.1 ~\rm cm^{-3}} $ & 100 pc & $1$ & 21.8 K\\
		EoSL10 & $3.3 \rm M_\odot \frac{n_H}{0.1 ~\rm cm^{-3}} $ & 10 pc & $1$ & 0.218 K\\
		\hline
	\end{tabular}
\end{table}
\end{comment}

\begin{comment}

The virial criteria therefore is a better physical motivation 
to use as compared to the temperature criterion.
The virial criterion is calculated as:
\begin{equation}
     \alpha \equiv \frac{\sigma_{3D}^2 + \sigma_{th}^2}{G \rho^{1/3} M_{res}^{2/3}} < \alpha_\text{vir}
\end{equation}
In which $\alpha$ is the virial criterion, $G$ is the gravitational constant, $\rho$ is the density and $M_\text{res}$ is the mass resolution, $\sigma_{3D}$ is the 3 dimensional velocity dispersion which we calculate in a SPH way as:
\begin{equation}
    \sigma_{3D}^2 = \frac{1}{\rho_i} \sum\limits_{j=1}^N m_j W(r_{ij}, h_i) |\mathbf{v}_i - \mathbf{v}_j|^2 
\end{equation}
and $\sigma_\text{th}$ is the thermal velocity dispersion given by:
\begin{equation}
    \sigma_{th}^2 = \sigma_{th,SPH}^2 \frac{T_{subgrid}}{T_{SPH}}
\end{equation}
which is identical to the SPH velocity dispersion:
\begin{equation}
    \sigma_{th, SPH}^2 = \frac{3 P}{\rho}
\end{equation}
when we are not on the EoS and lowered by the subgrid temperature over the SPH temperature when we are on the EoS.
\end{comment}
